Fair-by-design matching

Matching algorithms are used routinely to match donors to recipients for solid organs transplantation, for the assignment of medical residents to hospitals, record linkage in databases, scheduling jobs on machines, network switching, online advertising, and image recognition, among others. Although many optimal solutions may exist to a given matching problem, when the elements that shall or not be included in a solution correspond to individuals, it becomes of paramount importance that the solution be selected fairly. In this paper we study individual fairness in matching problems. Given that many maximum matchings may exist, each one satisfying a different set of individuals, the only way to guarantee fairness is through randomization. Hence we introduce the distributional maxmin fairness framework which provides, for any given input instance, the strongest guarantee possible simultaneously for all individuals in terms of satisfaction probability (the probability of being matched in the solution). Specifically, a probability distribution over feasible solutions is maxmin-fair if it is not possible to improve the satisfaction probability of any individual without decreasing it for some other individual which is no better off. In the special case of matchings in bipartite graphs, our framework is equivalent to the egalitarian mechanism of Bogomolnaia and Mouline. Our main contribution is a polynomial-time algorithm for fair matching building on techniques from minimum cuts, and edge-coloring algorithms for regular bipartite graphs, and transversal theory. For bipartite graphs, our algorithm runs in $O((|V|^2 + |E||V|^{2/3}) \cdot (\log |V|)^2)$ expected time and scales to graphs with tens of millions of vertices and hundreds of millions of edges. To the best of our knowledge, this provides the first large-scale implementation of the egalitarian mechanism.

==> generalizations.tex <==
%\note{I would call this Section \textbf{"Generalizations"} instead of "The General case".}
We discuss some
natural ways to generalize our algorithmic results from Section~\ref{sec:algorithms}.
%\textcolor[rgb]{0.00,0.00,1.00}{\textbf{our results}}.
The first deals with
matroid problems %which already made an appearance in Section~\ref{sec:properties}.
(see Section~\ref{sec:properties}).
For this we need an additional condition about the \emph{computational efficiency} of verifying the feasibility of a
candidate solution.

%\note{What does "our results" refer to? Algorithms in Section 4? Or the whole paper? We need to be more specific. Also, you're mentioning matroids, but these have been discussed before, so we need to throw some connections to what said in Section 3 and not introduce as this.}

%\enlargethispage{3\baselineskip}
\subsection{Efficiently encoded matroid problems}
Call a matroid problem \emph{efficiently encoded} if
    it admits a polynomial-time \emph{independence oracle}, which answers %is an algorithm answering %i.e., a polynomial-time algorithm for the
    the question:
%    \begin{center}
    ``given $X$ and $A \subseteq \calU$, is $A \in\calS$?''
%    \end{center}

%\note{What is the relation of these problems with Section 3?}

    Examples of efficiently encoded matroid problems include finding %\textcolor[rgb]{0.00,0.00,1.00}{e.g., }
    (a) sets of matchable vertices in a graph;
(b) linearly independent sets of columns in a matrix;
    (c) acyclic sets of edges in a graph; (d) sets of unit-length tasks (each with a given deadline) that
    may be scheduled on a single machine;
    (e) sets of vertices in a graph for which
    edge-disjoint paths from another specified vertex exist.
    \mycomment{
                %\paragraph{Examples of matroid problems:}
                \begin{itemize}
                    \item $X = (V, E)$ is an arbitrary graph, $\users{X} = V$ and and $T \subseteq V$ belongs to
                    $\solt{X}$ iff there is a
                    matching in $X$ covering $T$;
                %    \item $X$ is a collection of disjoint subsets of $V$, $\users{X} = V$ and $T \subseteq V$ belongs to $\solt{X}$ iff $T$ includes at most one element from each set in the collection.
                    \item $X$ is a finite-dimensional vector space, $L$ is its set of vectors and $T \subseteq L$
                    belongs to $\solt{X}$ iff $T$ is an independent set of vectors.
                    \item $X$ is a set of $n$ tasks. Each task takes one day to complete and
                    has an associated deadline.  $T\subseteq X$ belongs to $\solt{X}$ iff it is possible to schedule
                    all the tasks in $T$ at or before their respective deadlines.
                    \item $X = (V, E)$ is an arbitrary graph, $\users{X} = E$ and and $T \subseteq E$ belongs to
                    $\solt{X}$ iff the edges in $T$ form a tree;
                    \item $X = (G, s)$ is an arbitrary directed graph together with a fixed vertex $s\in V(G)$. $L = V$. A subset $T\subseteq L$ belongs to $\solt{X}$ iff there are edge-disjoint paths from $s$ to each element of $T$.
                %    \item certain scheduling problem of unit-tasks with deadlines (here $T$ is a set of tasks and belongs to $\solt{X}$ if they can all be scheduling together respecting the deadlines).
                %    \item A family of sets is laminar if any two sets are either disjoint or one is contained in the other. The sets that intersect at most $k(F)$ times for each set $F$ in the laminar family form a matroid.
                %    \item other: cycle basis, dual matroids, etc.
                \end{itemize}
    }

\ifhideproofs
\else
One may prove the existence of a fair decomposition analogous to
Theorem~\ref{thm:decomp}. The proof is analogous, except that it uses the submodularity and subadditivity properties of the rank function in place of those of the cardinality of the
neighborhood function.


Consider a matroid $M$ with ground set $L$.    For $A\subseteq L$, denote by $M\rst{A}$ the \emph{restriction} of $M$ to $A$,
i.e., the matroid
      $M\rst{A}$ with ground set $A$ and independent sets $M\rst{A} = \{ I \in M \mid I \subseteq A\}$.
      Denote by $M/A$ the \emph{contraction} of $M$ to $L \setminus A$, 
      i.e., the matroid $M/A$ with ground set $L \setminus A$ and rank function
      $\rho_{M/A}(X) = \rho(A \cup  X) - \rho(A).$
    For any subset $H\subseteq L$, let $\pi(H)$ (resp., $\Pi(H)$) be the minimum (resp., maximum)
    satisfaction probability of an element of $L$ in a maxmin-fair distribution.
{The set $X\subseteq L$ is \emph{fairly isolated} if $\Pi(G\rst{X}) < \pi(G/X)$ or $\Gamma(X) =
    \emptyset$ or $X = L$.}
\begin{mytheorem}[Fair decomposition of matroids]\label{thm:fair_matroids}
The fairly isolated sets in a matroid $M$ form a chain $$S_0 \subseteq S_1 \subseteq S_2 \ldots
\subseteq S_{k-1} \subseteq S_k = L$$ with respect to set inclusion.
Define $\lambda_0 = 0$ and  $$\lambda_i = \frac{ \rho(S_i) - \rho(S_{i-1}) }{|S_i-S_{i-1}|}.$$
The following properties hold:
%If $\lambda_i$ denotes the value of $S_i$, the following properties hold:
\begin{enumerate}[(a)]
    \item $S_0 = span(\emptyset)$ and $S_{i+1}$ is the unique maximal set $Y\supsetneq S_i$ minimizing $ \frac{ \rho(Y) - \rho(S_i) }{|Y \setminus S_i|}$.
%    \item $S_k = L$ and $S_{i-1}$ is the unique maximal set $Y \subsetneq S_i$ maximizing $ \frac{ \rho(S_i) - \rho(Y) }{|S_i \setminus Y|}$.
%    \item Each $S_i$ is closed, i.e., $span(S_i) = S_i$.
%    \item $0 = \lambda_0 \le \lambda_1 \le \ldots \le \lambda_{k} \le 1$.
    \item If $v \in S_i\setminus S_{i-1}$, then the coverage probability of $v$ in any maxmin-fair
     solution is $\lambda_i$.
%    \item $\displaystyle \lambda_1 = \min_{\substack{\emptyset\neq S\subseteq L}}{\frac{|\rho(S)|}{|S|}}$ is the maxmin coverage of $L$.
%    \item $\displaystyle \lambda_k = \max_{\substack{S\subsetneq L}}{\frac{|\rho(L)-\rho(S)|}{|L\setminus S|}}$ is the minmax coverage of $L$.
    \item The chain $L\setminus S_k \subseteq L \setminus S_{k-1} \subseteq \ldots L \setminus S_1
    \ldots L \setminus S_0$ is the fair decomposition of the dual matroid $M^*$.
\end{enumerate}
\end{mytheorem}
\fi

%This condition is enough to enable the efficient construction of maxmin-fair distributions:
This condition enables efficient maxmin-fair algorithms:
\begin{mytheorem}\label{thm:algo_matroids}
For any efficiently encoded matroid problem, there is a polynomial-time algorithm inducing a
maxmin-fair distribution.
\end{mytheorem}
\fullversion{
\begin{proof}
Since this result will be shown shortly to be a consequence of the more general
    Theorem~\ref{thm:fairness_P}, we only sketch the idea of how to generalize the steps of our fair matching algorithm from
Section~\ref{sec:algorithms}. (This technique is still interesting as it yields a more efficient algorithm for matroids that
        that implied by Theorem~\ref{thm:fairness_P}.)

%\spara{Obtaining a fair decomposition efficiently.}
\spara{\emph{Step 1: Finding a fair decomposition.}}
Given $S_0, \ldots, S_{i-1}$, to find $S_i$ we need to minimize $(\rho(X) - \rho(S_i-1)) / |X -
S_{i-1}|$. Write $S_i = S_{i-1} \cup B_i$.
    Note that $\rho(X) - \rho(S_{i-1}) = \rho_{M/S_{i-1}(X)}$. We can
build a polynomial-time independence oracle for the contracted matroid $M/S_{i-1}$. Thus finding the
next block reduces to minimizing $\rho_{M/S_{i-1}}(B) / |B|$ in the contracted matroid.
For notational convenience we may assume $i=1$ and $M/S_{i-1} = M$.

For any $\lambda$, determining the existence of a set
with $\rho(S) \le \lambda |S|$ is equivalent to determining whether the minimum of the submodular
function $f_\lambda(S) = \rho(S) - \lambda |S|$ is at most zero. The existence of an independence oracle implies a
polynomial-time algorithm to compute this function. Since submodular function minimization is solvable
in polynomial time~\cite{submodular_minimization}, we can determine if there is some set with
$f_\lambda(S) \le 0$.
There is a polynomial number of rational values for $\lambda$ with denominator
at most $|L|$. By performing binary search on the set of possible values for $\lambda$ (or trying
        all of them), we obtain in
polynomial time a set minimizing $\rho(X) / |X|$. The union of any two such sets also minimizes
$\rho(X) / |X|$ by the submodularity of the rank function $\rho$, hence by repeating this procedure as many times as needed we can find the maximal
set  $B$ minimizing this ratio.
Contracting the current matroid by $B$ and proceeding in the same way if $B\neq L$ we find a fair
decomposition in polynomial time.

\spara{\emph{Step 2: Obtaining a fair distribution for each block.}}
%\spara{Finding the maxmin-fair distribution.}
If we find fair distributions $D_1, \ldots, D_k$ so that each $D_i$ is maxmin-fair
for $(M/S_i)\rst{S_i-S_{i-1}}$, then the distribution of $\bigcup_{i=1}^k M_i$ where each $M_i$ is drawn from $D_i$ will be
   maxmin-fair. So again we can reduce the general case to the case where there is a single block
   and all elements have the same satisfaction probability $\lambda$ in the maxmin-fair
   distribution. To find the distribution of bases realizing the desired probabilities, we may use
   the idea behind the proof of Theorem~\ref{thm:hall}.

%Now we focus on computing the fairness parameter. Given $\lambda$, the fairness parameter is at least $\lambda$ iff the function $f_\lambda(S) = \rho(S) - \lambda |S|$ has a non-negative minimum. Schrijver gave an algorithm to minimize a submodular function defined on subsets of $A$  in time $O(n^6 + t \cdot n^5)$, where $n = |A|$ and $t$ is the time needed to evaluate the rank of a set.  Since there are only $n^2$ possibilities for the optimal $\lambda$ (it must be of the form $p/q$ with $0 \le p \le q$ and $q \le n$), we can perform binary search and find the optimal $\lambda$ in time $O((n^6 + t \cdot n^5) \log n)$.

%For an upper bound we may assume $t \ge n$. Then we found $\lambda^*$ in time $\widetilde{O}(t \cdot n^5)$, and a set $S$ with $\rho(S) = \lambda^* |S|$.  By trying to remove each element of $S$ and solving the new problem, we can find a \emph{minimal} set with this ratio in time $\widetilde{O}(t \cdot n^6)$.



    Suppose $\lambda = r / s$, where $r$ and $s$ are integers.
    Make $r$ disjoint copies of the ground set $L$, $L' = L \cup \ldots \cup L$.
    For any $S'\subseteq A$, let % $o(S')$ denote the original set of elements, i.e.,
        $o(S') = \{ a \mid (a, i) \in S' \}$.
    Define
    $ \rho'(S') = \rho(o(S)). $
    Then $\rho'$ is the rank function of a matroid because it satisfies
     (a)   $ 0 \le \rho'(S') \le |S'|, $
     (b)   $ S' \subseteq T' \implies \rho'(S') \le \rho'(T'), $
        and
     (c)   $ \rho'(S' \cup T') + \rho'(S' \cap T') \le \rho'(S) + \rho'(T), $.
        \mycomment{
    the following:
    \begin{itemize}
    \item
        $ 0 \le \rho'(S') \le |S'|, $
            because $\rho'(S') = \rho(o(S')) \le |o(S')| \le |S'|$.
            \item
        $ S' \subseteq T' \implies \rho'(S') \le \rho'(T'), $
            because $S' \subseteq T'$ implies $o(S') \subseteq o(T')$.
            \item
        $ \rho'(S' \cup T') + \rho'(S' \cap T') \le \rho'(S) + \rho'(T), $
            because
            \begin{align*}
                \rho'(S' \cup T') + \rho'(S' \cap T')
                &=   \rho(o(S' \cup T')) +   \rho(o(S' \cap T')) \\
                &=   \rho(o(S') \cup o(T')) + \rho(o(S' \cap T')) \\
                &\le \rho(o(S') \cup o(T')) + \rho(o(S') \cap o(T')) \\
                &\le \rho(o(S')) + \rho(o(T')) \\
                &=   \rho'(S') + \rho'(T').\\
            \end{align*}
    \end{itemize}
        }

    Since $|o(S')| \ge |S'| / r$,
    we have that for all $S'$, $\rho'(S') = \rho(o(S')) \ge \lambda o(S') = (r / s) o(S') \ge (1/s) |S'|$.
    Then
 Edmond's matroid partitioning algorithm~\cite{matroid_partition} may be used
    to partition $M'$ into $s$ $\rho'$-independent sets,
       and since element of $M$ has $r$ copies in $M'$, every element is included $r$ times among those $s$.
       By definition $\rho'$-independent sets do not include copies of the same element.
       Therefore we found $s$ bases so that each element of $L$ is included in exactly $r$ of t hem;
       picking one of them at random gives the desired maxmin-fair distribution.
       \end{proof}
}

\subsection{Efficiently optimizable problems}
The class of problems with efficiently samplable maxmin-fair distributions is
%turns out to be
much larger than that of efficiently-encoded matroid problems.
\mycomment{
                We show that, in a certain sense, the fair version of any problem is as easy as its optimization
                version.
                \mycomment{
                            For intuition, recall that a well-known characterization of matroids~\cite{matroids_greedy}
                            asserts that a downwards-closed set system $M$ is a matroid over $L$ if and only if,
                            for each assignment of non-negative real weights to each element of $L$, the greedy algorithm finds a
                            maximum-weight base of $M$.
                                Let us call a problem \emph{efficiently
                                optimizable} if there is a polynomial-time \emph{weight optimization oracle}algorithm which, given an
                            assignment of non-negative real weights to each element of $L$, returns a maximum-weight element of $M$.
                            We call the latter algorithm a \emph{weight optimization oracle}.
                            Efficiently encoded matroid problems correspond to the very special case where the weight
                            optimization oracle is provided by the simple greedy
                            algorithm.
                }
                Call a problem \emph{efficiently optimizable} if there is a polynomial-time \emph{weight
                    optimization oracle}: an algorithm which, given  a non-negative weight function defined on
                    $\calU$,
                   % an assignment of non-negative real weights to each element of $L$,
                    returns a maximum-weight element of $\calS$.
                Any weight optimization oracle may be used as an independence oracle.
                %by setting all the weights in a subset $S\subseteq L$ to 1. It can also find a maximum-sized element of $M$ with minimum weight, by replacing each weight $w_v$ with the weight $L-w_v$, where $L$ is a sufficiently large number.
                By a well-known characterization of matroids~\cite{matroids_greedy},
                efficiently encoded matroid problems correspond to the very special case where the weight
                optimization oracle is provided by the simple greedy algorithm.
}
We show that, in a specific sense, the fair version of \emph{any} problem is as easy as its optimization
version.
Call a problem \emph{efficiently optimizable} if there is a polynomial-time \emph{weight
    optimization oracle}: an algorithm $\calO$ which, given  a non-negative weight function defined on
    $\calU$,
    returns an element of $\calS$ of maximum weight sum.
    \fullversion{(Such an oracle may be used as an independence oracle.)}
%by setting all the weights in a subset $S\subseteq L$ to 1. It can also find a maximum-sized element of $M$ with minimum weight, by replacing each weight $w_v$ with the weight $L-w_v$, where $L$ is a sufficiently large number.
By a characterization of matroids~\cite{matroids_greedy},
efficiently encoded matroid problems comprise the special case where $\calO$
is provided by the simple greedy algorithm.

%\note{Can we provide examples of some of these problems?}
\begin{myexample}
The following two problems are not matroid problems, but are efficiently optimizable nonetheless:
\squishlist
\item Given a graph and two vertices $s$ and $t$, find the vertices in a shortest path from $s$ to $t$.
Indeed, given any assignment of weights to vertices, a shortest path of maximum weight may be found
by dynamic programming on the
directed acyclic graph of a breadth-first-search from $s$.
\item The maximum bipartite matching problem where $ \calU = E$, that is, users correspond to \emph{edges} (not vertices) in the graph.
Then, given an assignment of weights to edges, a maximum matching of maximum weight may be found by
finding a maximum-weight set of edges belonging to the intersection of two 1-uniform matroids, which can be solved in
polynomial time~\cite{lawler_book}.
\squishend
\end{myexample}

\mycomment{
\begin{myexample} An efficiently optimizable problem which is not a matroid problem is the following:
given a graph and two vertices $s$ and $t$, find the set of vertices in a shortest path between $s$ and $t$.
Indeed, given any assignment of weights to vertices, a shortest path of maximum weight may be found
by dynamic programming on the
directed acyclic graph of a breadth-first-search from $s$.
\end{myexample}

\begin{myexample}
Another efficiently optimizable problem which is not a matroid problem is
 is a bipartite matching problem where users correspond to \emph{edges} (not vertices) in the graph.
Then, given an assignment of weights to edges, a maximum matching of maximum weight may be
identified by
finding a maximum-weight set of edges belonging to the intersection of two 1-uniform matroids, which can be solved in
polynomial time.
\end{myexample}
}
%    \note{\small Why is this example interesting? Can we think about an applications in which nodes of a social networks (humans) have interest in being selected in the shortest path? Any other efficiently optimizable problem which smells more concrete? more real-world?  \textcolor[rgb]{0.00,0.00,1.00}{David: I think this is the easiest example for the moment, I wouldn't worry much about this.} }


As usual, we characterize the fairness parameter. Given
an assignment $W\colon L \to \reals^{\ge 0}$
%assignments $W, \alpha: L \to \reals^{\ge 0}$
and $A \subseteq L$, define $W(A) = \sum_{v \in A} W(v)$.% and $\langle W, \alpha \rangle = \sum_{v \in L} W(v) \alpha(v)$.
\begin{mytheorem}
For any %\textcolor[rgb]{0.00,0.00,1.00}{\textbf{finite problem}}
problem $\calS$, % and any $\alpha:L \to \reals^{+}$,
    the minimum satisfaction probability in the maxmin-fair distribution is
\begin{equation}\label{eq:generalW}
% \max_{D\in\Delta} \min_{v \in L} \frac{\cov{D}{v}}{\alpha(v)} = \min_{W\in{\mathcal W}_\alpha} \max_{S\in \calS} \frac{W(S)}{\langle W, \alpha \rangle},
 \max_{D\in\Delta}\; \min_{u \in L} {\cov{D}{u}} = \min_{W\in{\mathcal W}_\alpha} \max_{S\in \calS}
 \frac{W(S)}{W(L)},
\end{equation}
where
${\mathcal W} = \{W:L \to \reals^{\ge 0} \mid W(L) > 0\}$
%${\mathcal W}_\alpha = \{W:L \to \reals^{\ge 0} \mid \langle W,\alpha \rangle > 0$\}
and  $\Delta$ is the set of all distributions over $\calS$.

\end{mytheorem}
%\enlargethispage{3\baselineskip}
%\note{What is a "finite problem"? Where have you defined it?}

\ifhideproofs\else
\begin{proof}
By homogeneity we need only consider functions $W$ with $W(L) = 1$. %$\langle W, \alpha \rangle = 1$.
Just like in the proof of Theorem~\ref{thm:matroids}, the following two problems can be written as
linear programs which are duals of each other:

{
\small{
\begin{minipage}{.48\linewidth}
    \begin{equation}\label{lp:fair2}
    \begin{array}{rrclcl}
    \displaystyle \max & \displaystyle \min_{v\in L} \sum_{B \ni v} {p_B} \\
            \\
    \textrm{s.t.}
    & \displaystyle \sum_{S \in \mathcal{S}} p_B  & = & 1 &  \\
    & p_B    &\ge& 0 \\
    \end{array}
    \end{equation}
\end{minipage}%
\begin{minipage}{.48\linewidth}
    \begin{equation}\label{lp:zv2}
    \begin{array}{rrclcl}
    \displaystyle \min & \displaystyle \max_{S\in\mathcal{S}} \displaystyle \sum_{v \in S} w_v \\
            \\
    \textrm{s.t.}
    & \displaystyle \sum_{v \in L} w_v  & = & 1 &  \\
    & w_v &\ge& 0. \\
    \end{array}
    \end{equation}
\end{minipage}
}
}

The left-hand side of~\eqref{eq:generalW} is the optimum of Program~\eqref{lp:fair2}, and
its right-hand side is the optimum of Program~\eqref{lp:zv2}.
The result follows from linear programming duality.
\end{proof}
\fi
%For matroid problems, the weightings $W$ attaining equality in~\eqref{eq:generalW} are uniform over a subset of $L$, but this does not hold in the general case (consider the problem$\calS = \{ \{0\}, \{1,2\}, \{1,3\}, \{2,3\} \}$  and the optimal weighting given by $W(0) = \frac{2}{5}$ and $W(1) = W(2) = W(3) = \frac{1}{5}$).
%and an optimal distribution has $\Pr[\{0\}]=\frac{2}{5}$ and $\Pr[\{1,2\}] = \Pr[\{1,3\}] = \Pr[\{2,3\}] = \frac{1}{5}$.
Using~\eqref{eq:generalW} %and the ellipsoid algorithm~\cite{separation_oracle},
one may compute the satisfaction probabilities of a maxmin-fair distribution of an efficiently
optimizable problem in polynomial time. 
\ifhideproofs
\else
            \begin{mytheorem}\label{thm:fairness_P}
            For any efficiently optimizable problem, the satisfaction probabilities of a maxmin-fair
            distribution can be computed in polynomial time.
            \end{mytheorem}
            In this case, however, the connection between maxmin-fairness and minimizing social inequality is lost.
            %    The satisfaction probabilities of a maxmin-fair distribution can be computed efficiently for any efficiently optimizable problem.  (However, the connection between maxmin-fairness and minimizing social inequality is lost.) Moreover, we have:
            \begin{proof}
            Let $D$ be a maxmin-fair distribution. We maintain the invariant that we know the satisfaction probabilities $\alpha_v = D[v]$ for all $v$
            in a subset $K\subseteq L$, and that $\cov{D}{v} \ge \max_{w \in K} \alpha_w$.
            Initially $K = \emptyset$. We show how to augment $S$ in polynomial time, which gives the result.
            We take~\eqref{lp:fair2} and add constraints to express the required satisfaction probabilities for
            $K$, obtaining the primal program
            {
            \small{
                \begin{equation}\label{lp:fair3}
                \begin{array}{rrclcl}
                \displaystyle \max & \lambda \\
                        \\
                \textrm{s.t.}
                & \displaystyle \sum_{B \ni v} {p_B} & \ge & \alpha_v & \forall v \in K \\
                & \displaystyle \sum_{B \ni v} {p_B} - \lambda & \ge & 0 & \forall v \notin K \\
                & \displaystyle \sum_{S \in \mathcal{S}} p_B  & = & 1 &  \\
                & p_B    &\ge& 0 \\
                \end{array}
                \end{equation}
            }
            }
            and its dual
            {
            \small
            {
                \begin{equation}\label{lp:zv3}
                \begin{array}{rrclcl}
                \displaystyle \min & \displaystyle \left[ \max_{S\in\mathcal{S}} \displaystyle \sum_{v \in S}
                w_v\right] - \sum_{v \in K} \alpha_v w_v \\
                \textrm{s.t.}
                & \displaystyle \sum_{v \in L} w_v  & = & 1 &  \\
                & w_v &\ge& 0. \\
                \end{array}
                \end{equation}
            }
            }

            The dual~\eqref{lp:zv3} has $|L|$ variables but a
            possibly exponential number of constraints (one for each candidate solution $S$, plus the constraint
                    $\sum_v w_v = 1$). To get around this
            difficulty, observe that it has a separation oracle: given $\{w_v\}_{v \in L}$ and
            $\lambda \in \reals$, we can determine if the optimum of~\eqref{lp:zv3} is at most $\lambda$ by using the weight
            optimization oracle and answering
            ``yes'' if the weight of the solution is no larger than $\lambda + \sum_{v\in K} \alpha_v w_v$. Otherwise we answer ``no'' and we can
            detect a violated constraint, given either by the base found by the optimization oracle, or by the
            constraint $\sum_v w_v = 1$, which can be checked separately. The existence of a separation oracle
            implies the solvability of~\eqref{lp:zv3} in polynomial time via the ellipsoid algorithm, by a result of  Gr{\"o}tschel, Lov{\'a}sz and Schrijver~\cite{separation_oracle, ellipsoid_book}.

            Suppose now that the optimal dual solution found is given by $\{w_v\}$ and has optimum value $\lambda$.
            These variables are dual to $\{p_S\}$ in~\eqref{lp:fair2} and~\eqref{lp:zv2}.
                        By
                        complementary slackness, $w_v > 0$ implies that the corresponding constraint is tight:
                        $\sum_{B \ni v} p_B \ge \alpha_v$ if $v \in K$, and
            $\sum_{B \ni v} p_B = \lambda$ if $v \notin K$.
            Because $\cov{D}{v} \ge \max_{w \in K} \alpha_w$ by assumption, the set $K' = \{ v \notin K \mid
            w_v > 0\}$ is non-empty. Therefore we can add $K'$ to $K$ and repeat the process; we stop when $K = L$.
            The number of iterations is at most $L$, and each iteration runs in polynomial time.
            \end{proof}
\fi
Moreover, the distribution itself can be found:
\begin{mytheorem}\label{thm:general_algo}
For any efficiently optimizable search problem, there is a polynomial-time algorithm inducing a
maxmin-fair distribution  whose support size is polynomial in $|\calU|$.
%supported over $O(n^2 \log^2{n})$ solutions, where $n = |L|$.
\end{mytheorem}
%For insight about why Theorem~\ref{thm:general_algo} should be true, consider an adaptive weight scheme. Initially all weights are set to 1 (we have no preference for any user).
Why should Theorem~\ref{thm:general_algo} be true? Imagine an adaptive weight scheme initially setting all user
weights to 1.
Our weight optimization oracle $\calO$ gives a maximum-weight
solution. With a view to attaining maxmin-fairness, % constructing a maxmin-fair distribution, we
we reduce the
weight of the users included in this solution, and raise the rest. Now $\calO$ returns
a second solution. By suitably adjusting user weights to encourage including users that have
been too often unsatisfied (and the probability of each
solution returned) we may obtain a maxmin-fair distribution.

%Theorem~\ref{thm:general_algo}
%This may be viewed as an existential result; an efficient fair algorithm exists for any optimizable search problem, but the method implicit in the proof may lead to suboptimal running times, leaving the door open to further research on specific problems.
\ifhideproofs\else
\begin{proof}
Consider the pair of LP programs used in the last iteration in the proof of
Theorem~\ref{thm:fairness_P} (so that $K \cup K'=L$). We used the
separation oracle and the ellipsoid algorithm to solve LP~\eqref{lp:zv2}. Since all coefficients in
our LPs can be represented in a polynomial number of bits, the number $t$ of calls to the separation
oracle during the run of the ellipsoid algorithm can be bounded by a polynomial in the number of
variables $|L|$ % $t = O(n^2 \log^2{n})$
(see~\cite{ellipsoid_book}). Consider the subprogram of~\eqref{lp:zv3} formed by using only these
$t$ constraints, along with  $\sum_v w_v = 1$ and the non-negativity constraints. If we run the
ellipsoid algorithm  on the new subprogram instead, we will find the same solution.  Therefore the
reduced set of constraints is enough by itself to guarantee that the optimum of LP~\eqref{lp:zv3} is at least
$\lambda$ (hence exactly $\lambda$); all other constraints are redundant. The dual of this subprogram is a subprogram of the primal
LP~\eqref{lp:fair3} using only $t$ of the variables $p_B$ and having the same optimal value. Any
solution to this reduced primal program gives the desired distribution.
\end{proof}
\fi




\mycomment{
\subsection{Support size}
Consider an  graph with $\Gamma(0) = \Gamma(1) = a$ and $\Gamma(2) = \Gamma(3) = \Gamma(4) = b$.
The minmax solution has $cov(0) = cov(1) = 1/2$ and $cov(2) = cov(3) = cov(4) = 1/3$.
A uniform distribution needs to have support 6 at least. But there is a solution which uses fewer
matchings:
let $\Pr[02] = \Pr[13] = 1/3$ and $\Pr[04] = \Pr[14] = 1/6$. This works!

Also I think that the ellipsoid method implies that $O(n \log n)$ bases suffice.
And for approximations, $O(\log n / \lambda)$. (When $\lambda$ is of the order $1/n$ we need n
        matchings anyway.)

In the case of matchings I think $n$ matchings always suffice, because of Birkhoff-Von Neumann with
some phantom vertices: for each tight block $S$,  add $S - \rho(S)$ phantom vertices and edge
probabilities $1/n$ between each vertex and them.

How to obtain solutions like this?
Easy:
 first try to satisfy $0$. I can pick $02$, the maximum probability is $1/3$.
 Now $2$ is already taken.
 I still need another $1/6$ for $0$. So I pick $03$ with probability $1/6$.
 Now I have $1/6$ left for $3$ and $1$ left for $1$. So pick $13$ with probability $1/6$, and
 finally $1 4$ with probability $1/3$.
}

%\subsection{Optimization problems}

